Learning to Fly in Seconds

Learning-based methods, particularly Reinforcement Learning (RL), hold great promise for streamlining deployment, enhancing performance, and achieving generalization in the control of autonomous multirotor aerial vehicles. Deep RL has been able to control complex systems with impressive fidelity and agility in simulation but the simulation-to-reality transfer often brings a hard-to-bridge reality gap. Moreover, RL is commonly plagued by prohibitively long training times. In this work, we propose a novel asymmetric actor-critic-based architecture coupled with a highly reliable RL-based training paradigm for end-to-end quadrotor control. We show how curriculum learning and a highly optimized simulator enhance sample complexity and lead to fast training times. To precisely discuss the challenges related to low-level/end-to-end multirotor control, we also introduce a taxonomy that classifies the existing levels of control abstractions as well as non-linearities and domain parameters. Our framework enables Simulation-to-Reality (Sim2Real) transfer for direct RPM control after only 18 seconds of training on a consumer-grade laptop as well as its deployment on microcontrollers to control a multirotor under real-time guarantees. Finally, our solution exhibits competitive performance in trajectory tracking, as demonstrated through various experimental comparisons with existing state-of-the-art control solutions using a real Crazyflie nano quadrotor. We open source the code including a very fast multirotor dynamics simulator that can simulate about 5 months of flight per second on a laptop GPU. The fast training times and deployment to a cheap, off-the-shelf quadrotor lower the barriers to entry and help democratize the research and development of these systems.

==> tables/2_training_time.tex <==
\begin{table}[b!]
\def\arraystretch{1.3}
\centering
\begin{tabular}{c c c c c}
\hline
 Year & Name & Task & CPUs/GPUs & Time \\
\hline
\grayrow
 2016 & A2C \cite{mnih_asynchronous_2016} & MuJoCo & 16 / 0 & $24h$ \\
 2015 & GAE \cite{schulman_high-dimensional_2015} & 3D biped locomotion &  16 / 0 & $2h$ \\
\grayrow
 2015 & GAE \cite{schulman_high-dimensional_2015} & Quadruped locomotion & 32 / 0 & $4h$ \\
 2019 & PPO \cite{openai_solving_2019} & Rubik's cube & 29440 / 64 & $\sim 14d$ \\
\grayrow
 2021 & PPO \cite{kumar_rma_2021} & Quadruped locomotion & 8 / 1 & $24h$ \\
 2022 & PPO \cite{rudin_learning_2022} & Quadruped locomotion & 8 / 1 & $20m$ \\
\hline
\end{tabular}
\caption{Selected wall-clock training times for different algorithms and tasks}
\label{table:training_time}
\end{table}
